Unfolding Local Growth Rate Estimates for (Almost) Perfect Adversarial Detection

Convolutional neural networks (CNN) define the state-of-the-art solution on many perceptual tasks. However, current CNN approaches largely remain vulnerable against adversarial perturbations of the input that have been crafted specifically to fool the system while being quasi-imperceptible to the human eye. In recent years, various approaches have been proposed to defend CNNs against such attacks, for example by model hardening or by adding explicit defence mechanisms. Thereby, a small "detector" is included in the network and trained on the binary classification task of distinguishing genuine data from data containing adversarial perturbations. In this work, we propose a simple and light-weight detector, which leverages recent findings on the relation between networks' local intrinsic dimensionality (LID) and adversarial attacks. Based on a re-interpretation of the LID measure and several simple adaptations, we surpass the state-of-the-art on adversarial detection by a significant margin and reach almost perfect results in terms of F1-score for several networks and datasets. Sources available at: https://github.com/adverML/multiLID

==> utils/include.tex <==
\usepackage{wrapfig}

% If you use the following package, be sure to comment out \usepackate{xcolor}
% \usepackage[dvipsnames]{xcolor}

\usepackage{multirow,mathtools} \usepackage{algorithm,algpseudocode}

% Very useful for various special symbols
\usepackage{pifont}
% For \rowcolor
\usepackage{color, colortbl}

\usepackage{blindtext}
\usepackage{lipsum}
\usepackage{threeparttable}




%\usepackage[left=1in,right=1in,top=1in,bottom=1in]{geometry}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{times}
%\usepackage{arial}
\usepackage{multirow}
\usepackage{url}
%\usepackage{cite,subfigure,epsfig,epstopdf}
\usepackage{color}
\usepackage{xcolor}

\usepackage{enumitem}
% \usepackage{titlesec}
% \titleformat{\subsubsection}[runin]
%   {\normalfont\fontsize{11}{13}\bfseries}{\thesubsubsection}{1em}{}
\usepackage{xspace}
\usepackage{xfrac}
% \usepackage{tcolorbox}
\usepackage{comment}
\usepackage{tikz}
\usepackage{etoolbox}

\usepackage{placeins}
\usepackage{subcaption}


%%%%% SL
%
\definecolor{SL_color}{rgb}{0.858, 0.188, 0.478}
\newcommand{\SL}[1]{\textcolor{SL_color}{SL: #1}}
%\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
%\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\usepackage{pifont}
\usepackage{adjustbox}
\usepackage{threeparttable,booktabs}
\usepackage{multirow}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% \newcommand{\Def}[0]{\mathrel{\mathop:}=}
% \newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bphi}{\boldsymbol{\omega}}
% \newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\grad}{\nabla}

\DeclareMathOperator*{\ST}{\text{subject to}}

\usepackage{amsmath}%
\usepackage{MnSymbol}%
\usepackage{wasysym}%

% \usepackage{tcolorbox}

\usepackage{mathtools}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}


\usepackage{acro}



\usepackage{color, colortbl}
\definecolor{Gray}{gray}{0.93}
\definecolor{Orange}{rgb}{1,0.5,0}
\definecolor{DGray}{gray}{0.83}
\definecolor{LightCyan}{rgb}{0.88,1,1}


\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

% %\usepackage[most]{tcolorbox}
% \usepackage{{tcolorbox}}

